A $C^1$-continuous Trace-Finite-Cell-Method for linear thin shell analysis on implicitly defined surfaces

A Trace-Finite-Cell-Method for the numerical analysis of thin shells is presented combining concepts of the TraceFEM and the Finite-Cell-Method. As an underlying shell model we use the Koiter model, which we re-derive in strong form based on first principles of continuum mechanics by recasting well-known relations formulated in local coordinates to a formulation independent of a parametrization. The field approximation is constructed by restricting shape functions defined on a structured background grid on the shell surface. As shape functions we use on a background grid the tensor product of cubic splines. This yields $C^1$-continuous approximation spaces, which are required by the governing equations of fourth order. The parametrization-free formulation allows a natural implementation of the proposed method and manufactured solutions on arbitrary geometries for code verification. Thus, the implementation is verified by a convergence analysis where the error is computed with an exact manufactured solution. Furthermore, benchmark tests are investigated.

==> matlab_pics/gyroid_penalty.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.571\textwidth,
height=0.45\textwidth,
at={(0\textwidth,0\textwidth)},
scale only axis,
xmode=log,
xmin=1000000,
xmax=1e+18,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={$\text{penalty factor }\alpha$},
ymin=-6,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={$\text{displacement u}_\text{z}$},
axis background/.style={fill=white},
xmajorgrids,
xminorgrids,
ymajorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=1.8pt]
  table[row sep=crcr]{%
1400000	-3.7040235923849\\
2800000	-2.29664861272548\\
5600000	-1.57593361364869\\
11200000	-1.19556747586424\\
22400000	-0.985393128689339\\
44800000	-0.862096364158508\\
89600000	-0.784385333097716\\
179200000	-0.731602294210001\\
358400000	-0.692530055653679\\
716800000	-0.65923643057151\\
1433600000	-0.625225116729735\\
2867200000	-0.586823962189\\
5734400000	-0.544749496783694\\
11468800000	-0.502562753538065\\
22937600000	-0.463275319625272\\
45875200000	-0.428156447128712\\
91750400000	-0.397779234274934\\
183500800000	-0.372501857079024\\
367001600000	-0.352272815735091\\
734003200000	-0.336714462570389\\
1468006400000	-0.325099629523181\\
2936012800000	-0.316391691830894\\
5872025600000	-0.309444951291438\\
11744051200000	-0.303215513254864\\
23488102400000	-0.296976288291182\\
46976204800000	-0.290464216541834\\
93952409600000	-0.283936566289155\\
187904819200000	-0.278021953230609\\
375809638400000	-0.273239493807618\\
751619276800000	-0.269559366048883\\
1.5032385536e+15	-0.266500120037829\\
3.0064771072e+15	-0.263546073809356\\
6.0129542144e+15	-0.260140279538058\\
1.20259084288e+16	-0.254341486795326\\
2.40518168576e+16	-0.240122625762567\\
4.81036337152e+16	-0.195635046881528\\
9.62072674304e+16	-0.192229817857472\\
1.924145348608e+17	-0.195358713747639\\
3.848290697216e+17	-0.175372406932976\\
7.696581394432e+17	-0.159116293992992\\
};
\addlegendentry{ref. lev. = 1}

\addplot [color=mycolor2, line width=1.8pt]
  table[row sep=crcr]{%
1400000	-5.23727929109138\\
2800000	-3.82807225477098\\
5600000	-3.10779875244129\\
11200000	-2.72713605249241\\
22400000	-2.51014939177874\\
44800000	-2.37082663324897\\
89600000	-2.27057575985149\\
179200000	-2.19127230370885\\
358400000	-2.12032931622007\\
716800000	-2.04890121834449\\
1433600000	-1.97546129825285\\
2867200000	-1.9056582152747\\
5734400000	-1.84644114734683\\
11468800000	-1.80120128383727\\
22937600000	-1.76964612092381\\
45875200000	-1.74922157800255\\
91750400000	-1.73650882632477\\
183500800000	-1.72849459751531\\
367001600000	-1.72319550785175\\
734003200000	-1.71955455167803\\
1468006400000	-1.71701490082318\\
2936012800000	-1.71520506146547\\
5872025600000	-1.71383206696157\\
11744051200000	-1.71252757713406\\
23488102400000	-1.71125198962308\\
46976204800000	-1.70808778519746\\
93952409600000	-1.70546191869593\\
187904819200000	-1.70407648664821\\
375809638400000	-1.70179615594216\\
751619276800000	-1.70083646831884\\
1.5032385536e+15	-1.69703940109235\\
3.0064771072e+15	-1.69038549453223\\
6.0129542144e+15	-1.67010655978369\\
1.20259084288e+16	-1.65769153810308\\
2.40518168576e+16	-1.64475611549756\\
4.81036337152e+16	-1.63420999515768\\
9.62072674304e+16	-1.61457606400912\\
1.924145348608e+17	-1.21123710348712\\
3.848290697216e+17	-1.04743258406588\\
7.696581394432e+17	-0.552259062007377\\
};
\addlegendentry{ref. lev. = 2}

\addplot [color=mycolor3, line width=1.8pt]
  table[row sep=crcr]{%
1400000	-5.28772673370984\\
2800000	-3.88086794445027\\
5600000	-3.16272181880573\\
11200000	-2.78294290576012\\
22400000	-2.56510197061513\\
44800000	-2.42358605487352\\
89600000	-2.32062010095042\\
179200000	-2.23870802775808\\
358400000	-2.16590559401951\\
716800000	-2.09437995891932\\
1433600000	-2.02350259144269\\
2867200000	-1.95883766987181\\
5734400000	-1.90624861275491\\
11468800000	-1.86786606159393\\
22937600000	-1.8424730524536\\
45875200000	-1.82709879283117\\
91750400000	-1.81841860896865\\
183500800000	-1.81374257424858\\
367001600000	-1.81128999473204\\
734003200000	-1.81001871975488\\
1468006400000	-1.80936079124255\\
2936012800000	-1.80900399088286\\
5872025600000	-1.80880930045163\\
11744051200000	-1.80867855807105\\
23488102400000	-1.80861037232159\\
46976204800000	-1.80856950420408\\
93952409600000	-1.8084515721863\\
187904819200000	-1.80831546641788\\
375809638400000	-1.80813882432702\\
751619276800000	-1.80781937444598\\
1.5032385536e+15	-1.80766319537724\\
3.0064771072e+15	-1.80659848309482\\
6.0129542144e+15	-1.80299786184308\\
1.20259084288e+16	-1.79919321138746\\
2.40518168576e+16	-1.75546609158479\\
4.81036337152e+16	-1.4938652417771\\
9.62072674304e+16	-0.816506806150513\\
1.924145348608e+17	0.00287607871686\\
3.848290697216e+17	0.0168812614394919\\
7.696581394432e+17	0.0167241676952817\\
};
\addlegendentry{ref. lev. = 3}

\addplot [color=mycolor4, line width=1.8pt]
  table[row sep=crcr]{%
1400000	-5.28786591444056\\
2800000	-3.8810021060929\\
5600000	-3.16285170869084\\
11200000	-2.78306729597171\\
22400000	-2.5652193859989\\
44800000	-2.42369367870425\\
89600000	-2.32071658494868\\
179200000	-2.23879511091452\\
358400000	-2.16598739294169\\
716800000	-2.0944640380387\\
1433600000	-2.02359671082974\\
2867200000	-1.95894898131145\\
5734400000	-1.90637361097443\\
11468800000	-1.86800411412373\\
22937600000	-1.84262960190225\\
45875200000	-1.82726668361927\\
91750400000	-1.81859555122894\\
183500800000	-1.81393264429765\\
367001600000	-1.81149395660767\\
734003200000	-1.81023661655265\\
1468006400000	-1.80958759705807\\
2936012800000	-1.80925437491436\\
5872025600000	-1.80906948214604\\
11744051200000	-1.80897320743001\\
23488102400000	-1.80884500973257\\
46976204800000	-1.80876704419421\\
93952409600000	-1.80848547161786\\
187904819200000	-1.80592144745237\\
375809638400000	-1.80474662863096\\
751619276800000	-1.77296447634427\\
1.5032385536e+15	-1.70415555966228\\
3.0064771072e+15	-0.37629071042671\\
6.0129542144e+15	-0.188014649233705\\
1.20259084288e+16	-0.0976905002846438\\
2.40518168576e+16	-0.0431231150840597\\
4.81036337152e+16	-0.00337396558921776\\
9.62072674304e+16	0.00247505081721721\\
1.924145348608e+17	0.00387363567963761\\
3.848290697216e+17	0.00195487735489341\\
7.696581394432e+17	0.000475609663693555\\
};
\addlegendentry{ref. lev. = 4}

\addplot [color=black, line width=1.8pt]
  table[row sep=crcr]{%
1400000	-1.8812\\
2800000	-1.8812\\
5600000	-1.8812\\
11200000	-1.8812\\
22400000	-1.8812\\
44800000	-1.8812\\
89600000	-1.8812\\
179200000	-1.8812\\
358400000	-1.8812\\
716800000	-1.8812\\
1433600000	-1.8812\\
2867200000	-1.8812\\
5734400000	-1.8812\\
11468800000	-1.8812\\
22937600000	-1.8812\\
45875200000	-1.8812\\
91750400000	-1.8812\\
183500800000	-1.8812\\
367001600000	-1.8812\\
734003200000	-1.8812\\
1468006400000	-1.8812\\
2936012800000	-1.8812\\
5872025600000	-1.8812\\
11744051200000	-1.8812\\
23488102400000	-1.8812\\
46976204800000	-1.8812\\
93952409600000	-1.8812\\
187904819200000	-1.8812\\
375809638400000	-1.8812\\
751619276800000	-1.8812\\
1.5032385536e+15	-1.8812\\
3.0064771072e+15	-1.8812\\
6.0129542144e+15	-1.8812\\
1.20259084288e+16	-1.8812\\
2.40518168576e+16	-1.8812\\
4.81036337152e+16	-1.8812\\
9.62072674304e+16	-1.8812\\
1.924145348608e+17	-1.8812\\
3.848290697216e+17	-1.8812\\
7.696581394432e+17	-1.8812\\
};
\addlegendentry{reference}

\end{axis}
\end{tikzpicture}%

==> matlab_pics/roof2_results.tex <==
\begin{tabular}{lll}
null & Lagrange & penalty \\ 
\hline 
-0.30144 & -0.41987 & -0.28504 \\ 
-0.30214 & -0.30250 & -0.30213 \\ 
-0.30065 & 1.15175 & -0.30065 \\ 
-0.30060 & -0.30064 & -0.30060 \\ 
\hline 
\end{tabular}

==> matlab_pics/roof_penalty.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor5}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor6}{rgb}{0.30100,0.74500,0.93300}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.571\textwidth,
height=0.45\textwidth,
at={(0\textwidth,0\textwidth)},
scale only axis,
xmode=log,
xmin=8640,
xmax=4.74989023199232e+15,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={$\text{penalty factor }\alpha$},
ymin=-0.6,
ymax=0.1,
ylabel style={font=\color{white!15!black}},
ylabel={$\text{displacement u}_\text{z}$},
axis background/.style={fill=white},
xmajorgrids,
xminorgrids,
ymajorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=1.8pt]
  table[row sep=crcr]{%
8640	-0.566915344638285\\
17280	-0.424276741282727\\
34560	-0.368196197787768\\
69120	-0.334497730436558\\
138240	-0.331396663360062\\
276480	-0.397241229196968\\
552960	-0.304977258833875\\
1105920	-0.42283626412771\\
2211840	-0.349252643116976\\
4423680	-0.361448156001465\\
8847360	-0.305563542883052\\
17694720	-0.304018892682728\\
35389440	-0.302415647054417\\
70778880	-0.305567058958299\\
141557760	-0.299291940016005\\
283115520	-0.299424805229206\\
566231040	-0.299152335082425\\
1132462080	-0.299197639841252\\
2264924160	-0.29831340398824\\
4529848320	-0.29948117954144\\
9059696640	-0.296731709045792\\
18119393280	-0.296601961634582\\
36238786560	-0.29664315323248\\
72477573120	-0.291067265595567\\
144955146240	-0.296447723216005\\
289910292480	-0.296534291604752\\
579820584960	-0.287105548073171\\
1159641169920	-0.285343614375617\\
2319282339840	-0.284960825231716\\
4638564679680	-0.285196697414003\\
9277129359360	-0.284736661892175\\
18554258718720	-0.284473497426492\\
37108517437440	-0.285790862050339\\
74217034874880	-0.285313187523036\\
148434069749760	-0.281304357416263\\
296868139499520	-0.281167999504669\\
593736278999040	-0.278626551449606\\
1.18747255799808e+15	-0.274233244023042\\
2.37494511599616e+15	-0.267184186383887\\
4.74989023199232e+15	-0.222574980408778\\
};
\addlegendentry{ref. lev. = 1}

\addplot [color=mycolor2, line width=1.8pt]
  table[row sep=crcr]{%
8640	-0.552369450794709\\
17280	-0.430250327474755\\
34560	-0.369960421714769\\
69120	-0.339844013010502\\
138240	-0.324501066240355\\
276480	-0.316386278852763\\
552960	-0.311760761747859\\
1105920	-0.308772913646846\\
2211840	-0.30659351676181\\
4423680	-0.304963137121903\\
8847360	-0.30382735520651\\
17694720	-0.303105334871755\\
35389440	-0.302678433509571\\
70778880	-0.302434286285001\\
141557760	-0.302298185328707\\
283115520	-0.30222436243316\\
566231040	-0.302184975170772\\
1132462080	-0.302164120025673\\
2264924160	-0.302153272975729\\
4529848320	-0.302147501667899\\
9059696640	-0.302144522160156\\
18119393280	-0.302143012894497\\
36238786560	-0.302142217770282\\
72477573120	-0.302141984867013\\
144955146240	-0.302142171570067\\
289910292480	-0.302142312486158\\
579820584960	-0.302141902926731\\
1159641169920	-0.302142209010806\\
2319282339840	-0.302138168191013\\
4638564679680	-0.302138359005768\\
9277129359360	-0.302138735813847\\
18554258718720	-0.302128817118361\\
37108517437440	-0.302123617521437\\
74217034874880	-0.302149250726217\\
148434069749760	-0.302108552177869\\
296868139499520	-0.302243843346392\\
593736278999040	-0.302039472878216\\
1.18747255799808e+15	-0.297208414988038\\
2.37494511599616e+15	-0.301786995744175\\
4.74989023199232e+15	-0.299858404142351\\
};
\addlegendentry{ref. lev. = 2}

\addplot [color=mycolor3, line width=1.8pt]
  table[row sep=crcr]{%
8640	-0.555995949013192\\
17280	-0.433910351544699\\
34560	-0.373579378546992\\
69120	-0.343312888788234\\
138240	-0.327640788155641\\
276480	-0.318927302148829\\
552960	-0.313403169610298\\
1105920	-0.309363756844052\\
2211840	-0.306271563394322\\
4423680	-0.304054109918062\\
8847360	-0.302615264213953\\
17694720	-0.301751380279646\\
35389440	-0.301255698780794\\
70778880	-0.300978625490802\\
141557760	-0.300826754131772\\
283115520	-0.300744972171555\\
566231040	-0.300701574938901\\
1132462080	-0.300678340434398\\
2264924160	-0.300666292052673\\
4529848320	-0.300659978107252\\
9059696640	-0.300656734737927\\
18119393280	-0.300654927573\\
36238786560	-0.30065399815103\\
72477573120	-0.300654417230414\\
144955146240	-0.30065311528344\\
289910292480	-0.300652843059297\\
579820584960	-0.300652829542001\\
1159641169920	-0.300652845855152\\
2319282339840	-0.300655638402877\\
4638564679680	-0.300654382791317\\
9277129359360	-0.300660785549949\\
18554258718720	-0.300648794641147\\
37108517437440	-0.300658537369792\\
74217034874880	-0.300685402298935\\
148434069749760	-0.301139341670384\\
296868139499520	-0.300031895902388\\
593736278999040	-0.300421864750519\\
1.18747255799808e+15	-0.300189492253849\\
2.37494511599616e+15	-0.29842500593338\\
4.74989023199232e+15	-0.29488826531123\\
};
\addlegendentry{ref. lev. = 3}

\addplot [color=mycolor4, line width=1.8pt]
  table[row sep=crcr]{%
8640	-0.557149092830117\\
17280	-0.43504936327736\\
34560	-0.374687203068682\\
69120	-0.344360482083783\\
138240	-0.328580589407648\\
276480	-0.319695186040222\\
552960	-0.313943716369776\\
1105920	-0.309674062626704\\
2211840	-0.306411183537228\\
4423680	-0.304097488032025\\
8847360	-0.302611000582263\\
17694720	-0.301722520415652\\
35389440	-0.301212971669082\\
70778880	-0.300928345784868\\
141557760	-0.300772685059814\\
283115520	-0.30068906189203\\
566231040	-0.300644954901333\\
1132462080	-0.300621396588693\\
2264924160	-0.300609065428343\\
4529848320	-0.30060264607912\\
9059696640	-0.300598863605354\\
18119393280	-0.300596787406479\\
36238786560	-0.300596076587153\\
72477573120	-0.300598853099516\\
144955146240	-0.300596552934477\\
289910292480	-0.300602659855792\\
579820584960	-0.300597051656139\\
1159641169920	-0.300591584728093\\
2319282339840	-0.300599355196446\\
4638564679680	-0.300599064529621\\
9277129359360	-0.300606473459686\\
18554258718720	-0.300591494241785\\
37108517437440	-0.300576492109194\\
74217034874880	-0.300516242810238\\
148434069749760	-0.300388465903563\\
296868139499520	-0.299592897443503\\
593736278999040	-0.298444110625715\\
1.18747255799808e+15	-0.29510640278041\\
2.37494511599616e+15	-0.255310728999151\\
4.74989023199232e+15	-0.0690908863323444\\
};
\addlegendentry{ref. lev. = 4}

\addplot [color=mycolor5, line width=1.8pt]
  table[row sep=crcr]{%
8640	-0.557459363802838\\
17280	-0.435355266206933\\
34560	-0.374984382657343\\
69120	-0.344641191524624\\
138240	-0.328832113655177\\
276480	-0.319900792271612\\
552960	-0.314089963915604\\
1105920	-0.309762169951705\\
2211840	-0.306458039152625\\
4423680	-0.304122337862255\\
8847360	-0.302625509778142\\
17694720	-0.301731431433759\\
35389440	-0.301218220494642\\
70778880	-0.300930938564265\\
141557760	-0.300773515940109\\
283115520	-0.300688776142909\\
566231040	-0.300643686825799\\
1132462080	-0.300619820590081\\
2264924160	-0.30060714208525\\
4529848320	-0.300600431850842\\
9059696640	-0.300596838448989\\
18119393280	-0.300594930434044\\
36238786560	-0.300593873625062\\
72477573120	-0.300593569202679\\
144955146240	-0.300593379603667\\
289910292480	-0.300593677654666\\
579820584960	-0.300591980747693\\
1159641169920	-0.300598067437885\\
2319282339840	-0.30060009486175\\
4638564679680	-0.300473817105694\\
9277129359360	-0.299928504531199\\
18554258718720	-0.300382228484231\\
37108517437440	-0.300354162885954\\
74217034874880	-0.290153521811118\\
148434069749760	-0.276965380649884\\
296868139499520	-0.136027109610245\\
593736278999040	-0.0041243718667311\\
1.18747255799808e+15	-0.000272873399413389\\
2.37494511599616e+15	-0.00242921055594184\\
4.74989023199232e+15	0.00111332188338427\\
};
\addlegendentry{ref. lev. = 5}

\addplot [color=mycolor6, line width=1.8pt]
  table[row sep=crcr]{%
8640	-0.557650251913254\\
17280	-0.435542599764006\\
34560	-0.37516564861508\\
69120	-0.344811635762592\\
138240	-0.328983820622098\\
276480	-0.320023394174489\\
552960	-0.31417534731932\\
1105920	-0.309811522003266\\
2211840	-0.30648223784872\\
4423680	-0.304133571258517\\
8847360	-0.30263125172092\\
17694720	-0.301734903516409\\
35389440	-0.301220613191904\\
70778880	-0.300932724063013\\
141557760	-0.300774900422445\\
283115520	-0.300689840542064\\
566231040	-0.300644467151279\\
1132462080	-0.300620363208573\\
2264924160	-0.300607514886797\\
4529848320	-0.3006006355908\\
9059696640	-0.300596782492831\\
18119393280	-0.300598160113981\\
36238786560	-0.300598059861363\\
72477573120	-0.30061083914475\\
144955146240	-0.300493756274377\\
289910292480	-0.300440851970619\\
579820584960	-0.298701154707679\\
1159641169920	-0.299982175497384\\
2319282339840	-0.299422915170877\\
4638564679680	-0.263013346596734\\
9277129359360	-0.153073252712683\\
18554258718720	-0.0539700342772402\\
37108517437440	-0.0354563015732774\\
74217034874880	-0.0188267784529761\\
148434069749760	-0.00100236854760315\\
296868139499520	-0.00459243637347225\\
593736278999040	-0.00111582449529469\\
1.18747255799808e+15	-0.00128338615241038\\
2.37494511599616e+15	-0.000153988590014377\\
4.74989023199232e+15	-3.91082493510885e-05\\
};
\addlegendentry{ref. lev. = 6}

\addplot [color=black, line width=1.8pt]
  table[row sep=crcr]{%
8640	-0.3006\\
17280	-0.3006\\
34560	-0.3006\\
69120	-0.3006\\
138240	-0.3006\\
276480	-0.3006\\
552960	-0.3006\\
1105920	-0.3006\\
2211840	-0.3006\\
4423680	-0.3006\\
8847360	-0.3006\\
17694720	-0.3006\\
35389440	-0.3006\\
70778880	-0.3006\\
141557760	-0.3006\\
283115520	-0.3006\\
566231040	-0.3006\\
1132462080	-0.3006\\
2264924160	-0.3006\\
4529848320	-0.3006\\
9059696640	-0.3006\\
18119393280	-0.3006\\
36238786560	-0.3006\\
72477573120	-0.3006\\
144955146240	-0.3006\\
289910292480	-0.3006\\
579820584960	-0.3006\\
1159641169920	-0.3006\\
2319282339840	-0.3006\\
4638564679680	-0.3006\\
9277129359360	-0.3006\\
18554258718720	-0.3006\\
37108517437440	-0.3006\\
74217034874880	-0.3006\\
148434069749760	-0.3006\\
296868139499520	-0.3006\\
593736278999040	-0.3006\\
1.18747255799808e+15	-0.3006\\
2.37494511599616e+15	-0.3006\\
4.74989023199232e+15	-0.3006\\
};
\addlegendentry{reference}

\end{axis}
\end{tikzpicture}%
